Automatic sub-bundle tractometry reveals localized microstructural variations in complex white matter topographies

Conventional tractometry averages white matter microstructure into a single profile, masking intra-bundle spatial heterogeneity and diluting localized alterations. We propose an automatic sub-bundle tractometry framework using Fr{\'e}chet-based hierarchical clustering to decompose bundles into geometrically coherent sub-bundles, resolving complex fanning configurations without empirical thresholds. Multi-compartment metrics (fractional anisotropy, FA; isotropic free-water fraction, IFW) are projected onto these clusters. We evaluated this framework in 140 participants across early-life (ELD) and late-life (LLD) depression cohorts, alongside age-matched healthy controls. We assessed performance based on microstructural homogeneity, sensitivity to age, and clinical group differences. Proposed sub-bundle metrics were significantly more homogeneous than classical full bundle profiles (p < 0.001). Our approach showed enhanced sensitivity, detecting more age-correlated bundles in elderly controls (11 vs. 5) and more clinical group differences in LLD (FA: 6 vs. 4; IFW: 23 vs. 17) with larger effect sizes. In ELD, it improved the detection of subtle FA differences between remitted and resistant individuals (2.9% vs. 1.8%). Gains were particularly pronounced in LLD, reflecting the framework's ability to resolve fanning tracts susceptible to brain aging. By preserving spatial heterogeneity, this automatic decomposition provides a robust foundation for large-scale clinical tractometry.

==> results/homogeneity/summary/significance_summary_table.tex <==
\begin{tabular}{llcccccc}
 &  & \multicolumn{3}{c}{ELD} & \multicolumn{3}{c}{LLD} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
Metric & Test & $\text{Centerline}$ & $\text{Endpoints}$ & $\text{Fréchet}$ & $\text{Centerline}$ & $\text{Endpoints}$ & $\text{Fréchet}$ \\
\midrule
\multirow{3}{*}{FA} & Cluster heterogeneity (ANOVA) & 0 & 42 & \textbf{47} & 0 & 36 & \textbf{48} \\
 & Group discriminability (ANOVA) & 13 & 13 & \textbf{15} & 10 & 13 & \textbf{17} \\
 & Age correlation (Pearson) & 13 & 19 & \textbf{22} & 6 & 12 & \textbf{18} \\
\midrule
\multirow{3}{*}{IFW} & Cluster heterogeneity (ANOVA) & 0 & 38 & \textbf{44} & 0 & 32 & \textbf{34} \\
 & Group discriminability (ANOVA) & \textbf{2} & \textbf{2} & 1 & 23 & 22 & \textbf{31} \\
 & Age correlation (Pearson) & 2 & \textbf{6} & 4 & 41 & 39 & \textbf{46} \\
\bottomrule
\end{tabular}
